Analytics of Longitudinal System Monitoring Data for Performance Prediction

In recent years, several HPC facilities have started continuous monitoring of their systems and jobs to collect performance-related data for understanding performance and operational efficiency. Such data can be used to optimize the performance of individual jobs and the overall system by creating data-driven models that can predict the performance of jobs waiting in the scheduler queue. In this paper, we model the performance of representative control jobs using longitudinal system-wide monitoring data and machine learning to explore the causes of performance variability. We analyze these prediction models in great detail to identify the features that are dominant predictors of performance. We demonstrate that such models can be application-agnostic and can be used for predicting performance of applications that are not included in training.

==> Makefile <==
MAIN=paper

all: $(MAIN).pdf

$(MAIN).pdf: $(wildcard *.tex) $(wildcard *.tikz)
	pdflatex $(LATEXFLAGS) $(MAIN)
	bibtex $(MAIN)
	pdflatex $(LATEXFLAGS) $(MAIN)
	pdflatex $(LATEXFLAGS) $(MAIN)

clean:
	$(RM) *.aux *.log $(MAIN).dvi $(MAIN).ps $(MAIN).pdf $(MAIN).bbl $(MAIN).blg $(MAIN).synctex.gz

findref:
	@echo
	@test \
          `grep -c undefined $(MAIN).log | grep -v There | sed 's/.*\`//g' | sed "s/'.*//g"` = "0" \
            && echo "No undefined references" \
            || echo Finding undefined references ; \
               for uref in `grep undefined $(MAIN).log | grep -v There | sed 's/.*\`//g' | sed "s/'.*//g"`; \
               do  \
                echo "--> $$uref ";\
                grep -n "[rc][ei].*$$uref" *.tex | grep -v '.tex:[0-9]*:%' | sed 's/:/ -- Line /' | sed 's/:/:  /';\
                echo ;\
               done

.PHONY: clean


